Neutrino-Portal Dark Matter Detection Prospects at a Future Muon Collider

With no concrete evidence for non-gravitational interactions of dark matter to date, it is natural to wonder whether dark matter couples predominantly to the Standard Model (SM)'s neutrinos. Neutrino interactions (and the possible existence of additional neutrinophilic mediators) are substantially less understood than those of other SM particles, yet this picture will change dramatically in the coming decades with new neutrino sources. One potential new source arises with the construction of a high-energy muon collider (MuCol) -- due to muons' instability, a MuCol is a source of high-energy collimated neutrinos. Importantly, since the physics of muon decays (into neutrinos) is very well-understood, this leads to a neutrino flux with systematic uncertainties far smaller than fluxes from conventional high-energy (proton-sourced) neutrino beams. In this work, we study the capabilities of a potential neutrino detector, "MuCol$\nu$," placed ~100 m downstream of the MuCol interaction point. The MuCol$\nu$ detector would be especially capable of searching for a neutrinophilic mediator $\phi$ through the mono-neutrino scattering process $\nu_\mu N \to \mu^+ \phi X$, exceeding searches from other terrestrial approaches for $m_\phi$ in the ~few MeV -- ten GeV range. Even with a 10 kg-yr exposure, MuCol$\nu$ is capable of searching for well-motivated classes of thermal freeze-out and freeze-in neutrino-portal dark matter.

==> header.tex <==

\RequirePackage[colorlinks=true
,urlcolor=blue
,anchorcolor=blue
,citecolor=blue
,filecolor=blue
,linkcolor=blue
,menucolor=blue
,linktocpage=true
,pdfproducer=medialab
,pdfa=true
]{hyperref}

\usepackage{amsmath,amssymb,amsthm,amsfonts}
\usepackage{graphicx,tabularx}
\usepackage{color}
\usepackage{multirow}
\usepackage{comment}
\usepackage{enumitem}
\usepackage[capitalize]{cleveref}
\usepackage{slashed}
\usepackage[normalem]{ulem}
\usepackage{scalerel}
\usepackage{wrapfig}
\usepackage{cancel}
\usepackage{xcolor}
\usepackage{tikz-feynman}

\setlist[description]{leftmargin=0.3cm}
\setlist[itemize]{leftmargin=0.5cm}

\newcommand{\be}{\begin{equation} \begin{aligned}}
\newcommand{\ee}{\end{aligned} \end{equation}}
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}

\def\figureautorefname~#1\null{Fig.\,#1\null}
\def\tableautorefname~#1\null{Tab.\,#1\null}
\renewcommand{\sectionautorefname}{Sec.}
\renewcommand{\subsectionautorefname}{Sec.}
\def\equationautorefname~#1\null{Eq.\,(#1)\null}

% General symbols
\newcommand{\im}{\mathrm{i}}
\newcommand{\diff}{\mathrm{d}}
\newcommand{\eg}{{e.\,g.}~}
\newcommand{\ie}{{i.\,e.}~}
\newcommand{\equivalent}{\simeq}
\newcommand{\br}{\mathrm{BR}}

% Units
\newcommand{\ev}{\text{eV}}
\newcommand{\kev}{\text{keV}}
\newcommand{\mev}{\text{MeV}}
\newcommand{\gev}{\text{GeV}}
\newcommand{\tev}{\text{TeV}}

\newcommand{\ab}{\text{ab}}
\newcommand{\iab}{\text{ab}^{-1}}
\newcommand{\fb}{\text{fb}}
\newcommand{\ifb}{\text{fb}^{-1}}
\newcommand{\pb}{\text{pb}}
\newcommand{\ipb}{\text{pb}^{-1}}

\newcommand{\nm}{\text{nm}}
\newcommand{\micm}{\mu\text{m}}
\newcommand{\mm}{\text{mm}}
\newcommand{\cm}{\text{cm}}
\newcommand{\m}{\text{m}}
\newcommand{\km}{\text{km}}

\newcommand{\g}{\text{g}}
\newcommand{\kg}{\text{kg}}
\newcommand{\ton}{\text{t}}
\newcommand{\sr}{\text{sr}}
\newcommand{\ns}{\text{ns}}
\newcommand{\hz}{\text{Hz}}

%comments for changes
\RequirePackage[normalem]{ulem} 
\newcommand{\changed}[2]{{\protect\color{red}\sout{#1}}{\protect\color{blue}\uwave{#2}}}

% personalized comments
\newcommand{\Felix}[1]{\textcolor{magenta}{[FK: #1]}}
\newcommand{\st}[1]{\textcolor{orange}{[ST: #1]}}
\newcommand{\Jyotismita}[1]{\textcolor{red}{[JA: #1]}}
%\newcommand{\Felix}[1]{}
%\newcommand{\jlf}[1]{}

%\newcommand{\rem}[1]{}
\crefname{section}{Sec.}{Secs.}
\crefname{figure}{Fig.}{Figs.}
\crefname{equation}{Eq.}{Eqs.}
\crefname{table}{Table}{Tables}
\crefname{appendix}{Appendix}{Appendices}

% array
\renewcommand{\arraystretch}{1.2}

%Ref Style
\bibliographystyle{utphys}

% space on top/bottom from figures (copied from revtex)
\setcounter{topnumber}{2}
\def\topfraction{1}
\setcounter{bottomnumber}{1}
\def\bottomfraction{1}
\setcounter{totalnumber}{3}
\def\textfraction{0}
\def\floatpagefraction{1}
\setcounter{dbltopnumber}{2}
\def\dbltopfraction{1}
\def\dblfloatpagefraction{1}

\definecolor{nicegreen}{rgb}{0., 0.75, 0.46}
\newcommand{\KJK}[1]{{\bf \color{nicegreen} [KJK:  #1]}}

